Ollivier-Ricci Curvature of Riemannian Manifolds and Directed Graphs with Applications to Graph Neural Networks

This thesis is an exposition of Ollivier-Ricci Curvature of metric spaces as introduced by Yann Ollivier, which is based upon the 1-Wasserstein Distance and optimal transport theory. We present some of the major results and proofs that connect Ollivier-Ricci curvature with classical Ricci curvature of Riemannian manifolds, including extensions of various theoretical bounds and theorems such as Bonnet-Myers and Levy-Gromov. Then we shift to results introduced by Lin-Lu-Yau on an extension of Ollivier-Ricci curvature on graphs, as well as the work of Jost-Liu on proving various combinatorial bounds for graph Ollivier-Ricci curvature. At the end of this thesis we present novel ideas and proofs regarding extensions of these results to directed graphs, and finally applications of graph-based Ollivier-Ricci curvature to various algorithms in network science and graph machine learning.

==> endmatter/colophon.tex <==
%!TEX root = ../dissertation.tex
% Colophon (optional). Leave empty unless you want a final note.


==> endmatter/personalize.tex <==
%!TEX root = ../dissertation.tex


==> frontmatter/abstract.tex <==
%!TEX root = ../dissertation.tex
% the abstract


This thesis is an exposition of Ollivier-Ricci Curvature of metric spaces as introduced by Yann\linebreak[4] Ollivier, which is based upon the 1-Wasserstein Distance and optimal transport theory. We present some of the major results and proofs that connect Ollivier-Ricci curvature with classical Ricci curvature of Riemannian manifolds, including extensions of various theoretical bounds and theorems such as Bonnet-Myers and Levy-Gromov. Then we shift to results introduced by Lin-Lu-Yau on an extension of Ollivier-Ricci curvature on graphs,  as well as the work of Jost-Liu on proving various combinatorial bounds for graph Ollivier-Ricci curvature. At the end of this thesis we present novel ideas and proofs regarding extensions of these results to directed graphs, and finally applications of graph-based Ollivier-Ricci curvature to various algorithms in network science and graph machine learning. 

==> frontmatter/thanks.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

Thank you especially to Professor Melanie Weber who has advised me on this thesis and mentored me in the Geometric Machine Learning Group. She is to thank for encouraging me to pursue my interest graph curvature that began in her course APMTH220. Her prior research on Ollivier and Forman Ricci curvature was the original inspiration for this thesis and my interest this field. Thank you also to my secondary advisor Laura DeMarco for her encouragement and feedback during the writing of this thesis. I would like to thank Dr. Yu Tian for being a collaborator with Melanie and I on our research in the GeoML Group and in particular for sharing her expertise on directed graphs.

Additionally, in the Mathematics department I would like to express my immense gratitude for the phenomenal teaching of Dr. Puskar Mondal. His class on Semi-Riemannian Geometry was one of the highlights of my college experience. My love for geometry was discovered in his course. Thank you to Dr. Oliver Knill for being such an inspiring instructor of Differential Geometry when I was one of the course assistants this past fall. Your enthusiasm for differential geometry is contagious. I would also like to thank Professor Cliff Taubes for being so encouraging as an academic advisor in my early years at Harvard. In the Computer Science department, I would like to thank Professor Harry Lewis, Professor Todd Zickler, and Professor Michael Mitzenmacher for their inspiration and for deepening my love of applying mathematics to solve computational problems.

Thank you to the Eliot House community at Harvard for their constant support. Last but not least, I owe everything to my parents and siblings. Thank you for supporting my love of math and science.

%I would like to thank my roommates Jessica, Hannah, Mina, and Yanyan for always supporting me throughout college as well as the Eliot House community. Thank you to Rodney, Tyler, and Trace. Finally, thank you to my very large and loving family for their constant support throughout my academic journey. I would like to thank Mom and Dad to which I owe everything, including my love of science and learning. Thank you to my step-parents Mike and Clara, and my siblings Thomas, Clara, Nathan, Sadie, Finn, and Jack. This thesis is dedicated to my twin sister Clara for never wavering in her support for me, and for always being the one who pushes and inspires me the most.




